Accelerating Second-Order Differential Dynamic Programming for Rigid-Body Systems

This letter presents a method to reduce the computational demands of including second-order dynamics sensitivity information into the Differential Dynamic Programming (DDP) trajectory optimization algorithm. An approach to DDP is developed where all the necessary derivatives are computed with the same complexity as in the iterative Linear Quadratic Regulator (iLQR). Compared to linearized models used in iLQR, DDP more accurately represents the dynamics locally, but it is not often used since the second-order derivatives of the dynamics are tensorial and expensive to compute. This work shows how to avoid the need for computing the derivative tensor by instead leveraging reverse-mode accumulation of derivative information to compute a key vector-tensor product directly. We also show how the structure of the dynamics can be used to further accelerate these computations in rigid-body systems. Benchmarks of this approach for trajectory optimization with multi-link manipulators show that the benefits of DDP can often be included without sacrificing evaluation time, and can be done in fewer iterations than iLQR.

==> RNEAalgo.tex <==

% \begin{algorithm}[b]
% \caption{Recursive
% Newton-Euler algorithm as described by Featherstone~\cite{featherstone2014rigid}}
% \label{algo:RNEA}
% %\setstretch{1.2}
% \begin{algorithmic}[1]
% \REQUIRE $\q, \qd,\qdd, model$
% \STATE $\v_0 = 0, \a_0 = -\a_g$ 
% \STATE \underline{Forward Pass}
% \FOR{$i=1$ to $N$}
% \STATE $\v_i = \XM{i}{p(i)}\,\v_{p(i)}+\Pphi_i \,\qd_i$
% \STATE $\a_i = \XM{i}{p(i)}\, \a_{p(i)} + \crm{\v_i} \times \Pphi_i \qd_i + \Pphi_i \qdd_i$
% \STATE $\mathbfcal{F}_i= \I_i \a_i + \crm{\v_i} \I_i \v_i$
% \ENDFOR
% \STATE \underline{Backward Pass}
% \FOR{$i=N$ to $1$}
% \STATE $\t_i = \Pphi_i^T \mathbfcal{F}_i$
% \STATE $\mathbfcal{F}_{p(i)} = \mathbfcal{F}_{p(i)}  + \XM{i}{p(i)}^T \mathbfcal{F}_i $
% \ENDFOR
% \STATE Return $\t$
% \end{algorithmic}
% \label{alg:cor}
% \end{algorithm}



==> Resources/response_preamble.tex <==
\usepackage{scrextend}
\usepackage{color}
\usepackage{xr-hyper}
\usepackage[bookmarks=true,pdfborder={0 0 0}]{hyperref}
\usepackage{amsmath} 
\usepackage{amssymb}
\usepackage{Resources/qting}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{mathtools}
\usepackage{cmll}
\usepackage{cite}
\usepackage{subcaption}
\usepackage{stackengine}
\usepackage{scalerel}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{ifthen}
\usepackage{xcite}


%%% HELPER CODE FOR DEALING WITH EXTERNAL REFERENCES
\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}

\newcommand*{\addexternaldocument}[1]{
    \myexternaldocument{#1}
    \quotefrom{#1}
    \externalcitedocument{#1}
}
%%% END HELPER CODE

\usepackage{xcite}
\usepackage{nicefrac}
% correct bad hyphenation here




\usepackage{geometry}
 \geometry{
 a4paper,
 left=.95in,
 top=1in,
 bottom=1in,
 right=.95in
 }
 \usepackage{changepage}
 

\def\thesection{\arabic{section}}
\def\thesectiondis{}
\def\thesubsection{}
\def\thesubsectiondis{}

\newcounter{commentctr}[section]
%\newcounter{aecommentctr}[section]



%[R\thesection.\arabic{commentctr}]
\def\thecommentctr{(\thesection.\arabic{commentctr})}
\def\thecommentctrdis{\ifthenelse{\thesection = 0}{(AE.\arabic{commentctr}) Associate Editor:}{(R\thesection.\arabic{commentctr}) Reviewer:}}
\newcommand{\reviewer}[1]{\section{Reviewer #1}\setcounter{section}{#1}{\hrule height 1.5pt}\vspace{2mm}}


%\def\theaecommentctr{(\thesection.\arabic{commentctr})}
%\def\theaecommentctrdis{(\thesection.\arabic{commentctr}) AE:}

\newcommand{\associateeditor}{\section{Associate Editor}\setcounter{section}{0}{\hrule height 1.5pt}\vspace{2mm}}


\newcommand{\reviewsec}[1]{ \vspace{2mm} { #1} \vspace{1mm} {\hrule height .5pt}\vspace{2mm}}

\newenvironment{comment} {\par\refstepcounter{commentctr}{\bf\thecommentctrdis} \em} {}

\newenvironment{response}{\par\vspace{1.5mm} \begin{adjustwidth}{.5cm}{.5cm} }{ \end{adjustwidth}\vspace{5mm}}
    
\newcommand{\bc}{\begin{comment}
}
\newcommand{\ec}{\end{comment}}

\newcommand{\br}{\begin{response}
}
\newcommand{\er}{\end{response}}
\usepackage{setspace}

\newenvironment{quoted}{\vspace{1ex}\begin{addmargin}[2.5em]{0em}}{\end{addmargin}\vspace{1ex}}

\setlength{\parskip}{1ex} % 1ex plus 0.5ex minus 0.2ex}
\setlength{\parindent}{0pt}
\newcommand{\quickquote}[1]{ \vspace{1ex} \begin{quoted} \quotedisplay{#1} \end{quoted} \vspace{1ex} }

\newcommand{\red}[1]{#1}
\newcommand{\rev}[1]{{\color{blue}#1}}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> todo.tex <==





--running--- 


Keep fig 6 for now but run n=15

----done---
- Rerun Fig. 6 - And ensure accauracy of statements at end of section IV

-ModRNEA vs RNEA rerun;; Both ABA calls. 
% Revise red statement in conclusion as needed.

:) Run n =7 for fig 1 and fig 5

:) Font size in figures - Done

:) Update equations numbers in the figures to match their final numberings - done

:) coloring of plots - done 

:) Update Figures in review response to match final versions - done

